FETV: A Benchmark for Fine-Grained Evaluation of Open-Domain Text-to-Video Generation

Recently, open-domain text-to-video (T2V) generation models have made remarkable progress. However, the promising results are mainly shown by the qualitative cases of generated videos, while the quantitative evaluation of T2V models still faces two critical problems. Firstly, existing studies lack fine-grained evaluation of T2V models on different categories of text prompts. Although some benchmarks have categorized the prompts, their categorization either only focuses on a single aspect or fails to consider the temporal information in video generation. Secondly, it is unclear whether the automatic evaluation metrics are consistent with human standards. To address these problems, we propose FETV, a benchmark for Fine-grained Evaluation of Text-to-Video generation. FETV is multi-aspect, categorizing the prompts based on three orthogonal aspects: the major content, the attributes to control and the prompt complexity. FETV is also temporal-aware, which introduces several temporal categories tailored for video generation. Based on FETV, we conduct comprehensive manual evaluations of four representative T2V models, revealing their pros and cons on different categories of prompts from different aspects. We also extend FETV as a testbed to evaluate the reliability of automatic T2V metrics. The multi-aspect categorization of FETV enables fine-grained analysis of the metrics' reliability in different scenarios. We find that existing automatic metrics (e.g., CLIPScore and FVD) correlate poorly with human evaluation. To address this problem, we explore several solutions to improve CLIPScore and FVD, and develop two automatic metrics that exhibit significant higher correlation with humans than existing metrics. Benchmark page: https://github.com/llyx97/FETV.

==> tables/auto_human_correlation_static_quality.tex <==
\begin{table}[htbp]
\centering
\caption{Ranking of the models based on human evaluation of static quality (SQ), FID and FVD, on different spatial major contents. The inconsistent rankings with humans are marked in red. Full results of all categories and standard deviations are reported in the Appendix.}
\label{tab:auto_human_correlation_static_quality}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{@{}lcccccccccccc@{}}
\toprule
            & \multicolumn{3}{c}{\textbf{People}}                                        & \multicolumn{3}{c}{\textbf{Scenery}}                        & \multicolumn{3}{c}{\textbf{Artifacts}}                                      & \multicolumn{3}{c}{\textbf{Vehicles}}                                     \\ \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}
            & SQ     & FID $\downarrow$               & FVD $\downarrow$                 & SQ     & FID $\downarrow$                & FVD $\downarrow$ & SQ     & FID $\downarrow$                & FVD $\downarrow$                 & SQ     & FID $\downarrow$               & FVD $\downarrow$                \\ \midrule
T2V-zero    & 3.9(1) & {\color[HTML]{FE0000} 98.5(3)} & {\color[HTML]{FE0000} 757.0(2)}  & 4.4(1) & {\color[HTML]{FE0000} 109.2(2)} & 671.8(1)         & 4.0(1) & {\color[HTML]{FE0000} 109.0(2)} & {\color[HTML]{FE0000} 901.2(2)}  & 4.0(1) & {\color[HTML]{FE0000} 94.7(3)} & 676.2(1)                        \\
VideoFusion & 3.4(2) & {\color[HTML]{FE0000} 95.1(2)} & {\color[HTML]{FE0000} 1019.5(3)} & 4.2(2) & {\color[HTML]{FE0000} 100.7(1)} & 702.8(2)         & 3.6(2) & {\color[HTML]{FE0000} 113.3(3)} & {\color[HTML]{FE0000} 1449.7(3)} & 3.7(2) & {\color[HTML]{FE0000} 91.6(2)} & {\color[HTML]{FE0000} 798.9(3)} \\
CogVideo    & 3.1(3) & {\color[HTML]{FE0000} 87.0(1)} & {\color[HTML]{FE0000} 744.1(1)}  & 3.6(3) & 110.4(3)                        & 729.8(3)         & 3.1(3) & {\color[HTML]{FE0000} 103.0(1)} & {\color[HTML]{FE0000} 877.6(1)}  & 3.0(3) & {\color[HTML]{FE0000} 80.7(1)} & {\color[HTML]{FE0000} 643.2(2)} \\ \bottomrule
\end{tabular}
\end{adjustbox}
\end{table}

==> tables/auto_human_correlation_static_quality_app.tex <==
\begin{table}[htbp]
\centering
\caption{Ranking of the models based on human evaluation of static quality (SQ), FID and FVD, on different spatial major contents. The inconsistent rankings with humans are marked in red.}
\subfigure[Ranking on "Animals" and "Plants".]{
\centering
\resizebox{.6\textwidth}{!}{$
    \begin{tabular}{@{}llccccc@{}}
    \toprule
                & \multicolumn{3}{c}{\textbf{Animals}}                                       & \multicolumn{3}{c}{\textbf{Plants}}                         \\ \midrule
                & SQ     & FID $\downarrow$                & FVD $\downarrow$                & SQ     & FID $\downarrow$ & FVD $\downarrow$                \\ \midrule
    T2V-zero    & 4.0(1) & {\color[HTML]{FE0000} 127.2(3)} & {\color[HTML]{FE0000} 773.7(2)} & 4.5(1) & 120.7(1)         & {\color[HTML]{FE0000} 793.4(2)} \\
    VideoFusion & 3.7(2) & 118.9(2)                        & {\color[HTML]{FE0000} 791.7(3)} & 4.2(2) & 121.3(2)         & {\color[HTML]{FE0000} 709.5(1)} \\
    CogVideo    & 3.0(3) & {\color[HTML]{FE0000} 103.1(1)} & {\color[HTML]{FE0000} 762.8(1)} & 3.6(3) & 124.6(3)         & 808.1(3)                        \\ \bottomrule
    \end{tabular}
$}
}
\quad
\subfigure[Ranking on "Buildings", "Food" and "Illustrations".]{
\centering
\resizebox{.9\textwidth}{!}{$
    \begin{tabular}{@{}lllccccccc@{}}
    \toprule
                & \multicolumn{3}{c}{\textbf{Buildings}}                                     & \multicolumn{3}{c}{\textbf{Food}}                                           & \multicolumn{3}{c}{Illustrations}                                           \\ \midrule
                & SQ     & FID $\downarrow$                & FVD $\downarrow$                & SQ     & FID $\downarrow$                & FVD $\downarrow$                 & SQ     & FID $\downarrow$                & FVD $\downarrow$                 \\ \midrule
    T2V-zero    & 4.1(1) & {\color[HTML]{FE0000} 100.6(2)} & {\color[HTML]{FE0000} 729.1(2)} & 4.3(1) & {\color[HTML]{FE0000} 107.7(2)} & {\color[HTML]{FE0000} 1135.4(2)} & 3.7(1) & {\color[HTML]{FE0000} 174.8(2)} & {\color[HTML]{FE0000} 1708.6(2)} \\
    VideoFusion & 3.8(2) & {\color[HTML]{FE0000} 100.9(3)} & {\color[HTML]{FE0000} 764.0(3)} & 3.9(2) & {\color[HTML]{FE0000} 108.1(3)} & {\color[HTML]{FE0000} 1448.5(3)} & 3.5(2) & {\color[HTML]{FE0000} 194.7(3)} & {\color[HTML]{FE0000} 2667.2(3)} \\
    CogVideo    & 3.3(3) & {\color[HTML]{FE0000} 97.8(1)}  & {\color[HTML]{FE0000} 684.3(1)} & 3.2(3) & {\color[HTML]{FE0000} 100.7(1)} & {\color[HTML]{FE0000} 1045.6(1)} & 2.8(3) & {\color[HTML]{FE0000} 133.7(1)} & {\color[HTML]{FE0000} 869.8(1)}  \\ \bottomrule
    \end{tabular}
$}
}
\centering
\label{tab:auto_human_correlation_static_quality_app}
\end{table}

==> tables/auto_human_correlation_temporal_bak.tex <==
\begin{table}[t]
\centering
\caption{Ranking of the models based on human evaluation of temporal quality (TQ), FID and FVD, on different temporal major contents. The inconsistent rankings with humans are marked in red.}
\label{tab:auto_human_correlation_temporal_quality}
\resizebox{\textwidth}{!}{$
\begin{tabular}{lcccccccccccc}
\toprule
                & \multicolumn{3}{c}{\textbf{Fluid Motions}}                                 & \multicolumn{3}{c}{\textbf{Light Change}}                                   & \multicolumn{3}{c}{\textbf{Actions}}                                       & \multicolumn{3}{c}{\textbf{Kinetic Motions}}                               \\ \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} 
                & TQ     & FID $\downarrow$                            & FVD $\downarrow$                            & TQ     & FID $\downarrow$                            & FVD $\downarrow$                             & TQ     & FID $\downarrow$                            & FVD $\downarrow$                            & TQ     & FID $\downarrow$                            & FVD $\downarrow$                            \\ \midrule
VideoFusion     & 4.4(1) & {\color[HTML]{FE0000} 114.8(2)} & {\color[HTML]{FE0000} 991.0(3)} & 4.3(1) & {\color[HTML]{FE0000} 125.9(3)} & {\color[HTML]{FE0000} 1128.6(3)} & 3.8(1) & {\color[HTML]{FE0000} 101.7(3)} & {\color[HTML]{FE0000} 901.8(3)} & 4.0(1) & {\color[HTML]{FE0000} 103.1(2)} & {\color[HTML]{FE0000} 924.3(3)} \\
CogVideo        & 3.5(2) & {\color[HTML]{FE0000} 106.0(1)} & {\color[HTML]{FE0000} 742.8(1)} & 3.6(2) & {\color[HTML]{FE0000} 113.0(1)} & {\color[HTML]{FE0000} 676.0(1)}  & 3.2(2) & {\color[HTML]{FE0000} 90.0(1)}  & 714.8(2)                        & 3.2(2) & {\color[HTML]{FE0000} 93.1(1)}  & {\color[HTML]{FE0000} 666.6(1)} \\
Text2Video-zero & 2.0(3) & 115.3(3)                        & {\color[HTML]{FE0000} 800.5(2)} & 2.1(3) & {\color[HTML]{FE0000} 120.9(2)} & {\color[HTML]{FE0000} 891.7(2)}  & 2.0(3) & {\color[HTML]{FE0000} 100.2(2)} & {\color[HTML]{FE0000} 691.0(1)} & 2.0(3) & 103.5(3)                        & {\color[HTML]{FE0000} 726.8(2)} \\ \bottomrule
\end{tabular}
$}
\end{table}

==> tables/auto_human_correlation_temporal_quality.tex <==
\begin{table}[htbp]
\centering
\caption{Ranking of the models based on human evaluation of temporal quality (TQ), FID and FVD, on different temporal major contents. The inconsistent rankings with humans are marked in red.}
\label{tab:auto_human_correlation_temporal_quality}
\resizebox{\textwidth}{!}{$
\begin{tabular}{@{}lcccccccccccc@{}}
\toprule
                & \multicolumn{3}{c}{\textbf{Fluid Motions}}                                  & \multicolumn{3}{c}{\textbf{Light Change}}                                   & \multicolumn{3}{c}{\textbf{Actions}}                                       & \multicolumn{3}{c}{\textbf{Kinetic Motions}}                               \\ \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} 
                & TQ     & FID $\downarrow$                & FVD $\downarrow$                 & TQ     & FID $\downarrow$                & FVD $\downarrow$                 & TQ     & FID $\downarrow$                & FVD $\downarrow$                & TQ     & FID $\downarrow$                & FVD $\downarrow$                \\ \midrule
VideoFusion     & 4.4(1) & {\color[HTML]{FE0000} 114.8(2)} & {\color[HTML]{FE0000} 1125.1(3)} & 4.3(1) & {\color[HTML]{FE0000} 125.9(3)} & {\color[HTML]{FE0000} 1128.6(3)} & 3.8(1) & {\color[HTML]{FE0000} 101.7(3)} & {\color[HTML]{FE0000} 968.2(3)} & 4.0(1) & {\color[HTML]{FE0000} 103.1(2)} & {\color[HTML]{FE0000} 924.3(3)} \\
CogVideo        & 3.5(2) & {\color[HTML]{FE0000} 106.0(1)} & {\color[HTML]{FE0000} 671.1(1)}  & 3.6(2) & {\color[HTML]{FE0000} 113.0(1)} & {\color[HTML]{FE0000} 614.2(1)}  & 3.2(2) & {\color[HTML]{FE0000} 90.0(1)}  & 694.3(2)                        & 3.2(2) & {\color[HTML]{FE0000} 93.1(1)}  & {\color[HTML]{FE0000} 668.1(1)} \\
Text2Video-zero & 2.0(3) & 115.3(3)                        & {\color[HTML]{FE0000} 947.5(2)}  & 2.1(3) & {\color[HTML]{FE0000} 120.9(2)} & {\color[HTML]{FE0000} 878.7(2)}  & 2.0(3) & {\color[HTML]{FE0000} 100.2(2)} & {\color[HTML]{FE0000} 691.0(1)} & 2.0(3) & 103.5(3)                        & {\color[HTML]{FE0000} 754.3(2)} \\ \bottomrule
\end{tabular}
$}
\end{table}

==> tables/auto_human_t2v_ranking.tex <==
\begin{table}[t]
\centering
\caption{\add{Ranking of the models based on video-text alignment. The inconsistent rankings with humans are marked in red. Rankings under specific categories are reported in the Appendix.}}
\label{tab:auto_human_t2v_ranking}
\begin{adjustbox}{max width=0.8\textwidth}
\begin{tabular}{@{}llll ll@{}}
\toprule
             & Ground-Truth                    & VideoFusion                     &ZeroScope           & T2V-Zero                        & CogVideo \\ \midrule
CLIPScore    & {\color[HTML]{FE0000} 0.306(2)} & {\color[HTML]{FE0000} 0.315(1)} & 0.291(4) & 0.304(3)                 & 0.285(5) \\
CLIPScore-ft & 0.293(1) & {\color[HTML]{FE0000} 0.278(3)} & 0.274(4) & {\color[HTML]{FE0000} 0.285(2)} & 0.241(5) \\
BLIPScore    & {\color[HTML]{FE0000} 0.447(4)} & {\color[HTML]{FE0000} 0.471(1)} & 0.449(3) & {\color[HTML]{FE0000} 0.462(2)} & 0.411(5) \\
UMTScore     & 2.780(1)                        & 2.496(2)                        & 2.362(3) & 2.181(4)               & 1.023(5) \\ \midrule
Human        & 4.887(1)                        & 3.787(2)                        & & 3.416(3)                        & 3.103(4) \\ \bottomrule
\end{tabular}
\end{adjustbox}
\end{table}

==> tables/element_extraction_prompt.tex <==
\begin{table}
    \caption{Prompt for Element Extraction.}
    \label{tab:element_extract_prompt}
    \centering
    \begin{tcolorbox}
        Extract all key elements from the video description. Please ensure that your response contains extracted elements and follows the format of the following examples. If a phrase involves an object and an attribute, extract it as two elements. For example, extract white dog as white and dog.
        \\
        
        Description: kids are learning how to wrestle \\
        Elements: kids, learning, wrestle  \\

        Description: A white dog is running    \\
        Elements: white, dog, running \\

        Description: two men covered with snow hugging each other \\
        Elements: two, men, covered, snow, hugging \\

        Description: Backside view of woman butt in black leather skirt walking on street, close up, slow motion.  \\
        Elements: Backside view, woman, butt, black, leather skirt, walking, street, close up, slow motion  \\
    
        Description: Timelapse of a cityspace at sunset, aerial view \\
        Elements: Timelapse, cityspace, sunset, aerial view  \\
    
        Description: A small car driving to the right side of the road. \\
        Elements: small, car, driving, right side, road  \\

        Description: {\color[HTML]{0000FE} video\_description\_to\_extract\_elements}  \\
        Elements: 
        
    \end{tcolorbox}
\end{table}

==> tables/question_generation_prompt.tex <==
\begin{table}
    \caption{Prompt for Video QA Question Generation.}
    \label{tab:question_gen_prompt}
    \centering
    \begin{tcolorbox}
        Given a video description and extracted elements, generate two yes-no questions about each element. The answer of one question should be yes, and the answer of another question should be no. Ensure that the question can be answered based on information in the video description. Please ensure that the response follows the format of the following examples.
        \\
        
        Description: kids are learning how to wrestle \\
        Elements: kids, learning, wrestle \\
        About kids:  \\
        Q: are there kids?\\
        A: yes\\
        Q: are there cats?\\
        A: no\\
        About learning:\\
        Q: are the kids learning wrestling?\\
        A: yes\\
        Q: are the kids teaching wrestling?\\
        A: no\\
        About wrestle:\\
        Q: are the kids wrestling?\\
        A: yes\\
        Q: are the kids playing basketball?\\
        A: no\\

        {\color[HTML]{0000FE} more\_examples} \\

        Description: {\color[HTML]{0000FE} video\_description\_to\_extract\_elements}  \\
        Elements: {\color[HTML]{0000FE} extracted\_elements} \\
        About {\color[HTML]{0000FE} first\_element}:
        
    \end{tcolorbox}
\end{table}

==> tables/temporal_attribute.tex <==
\begin{table*}[t]
\centering
\caption{Descriptions and examples of temporal categories under the ``attribute control'' aspect.}
\label{tab:temporal_attribute}
\resizebox{\textwidth}{!}{$
\begin{tabular}{lll}
\toprule
Category                  & \multicolumn{1}{c}{Description}                        & \multicolumn{1}{c}{Example Prompts}                                                                                                                                                                      \\ \midrule
\textbf{Speed}            & Prompts that involve control over speed.               & \textit{\makecell{the cars drove fast; \\ bees flying, slow motion shot}}                                                                                            \\
                          &                                                        &                                                                                                                                                                                                   \\
\textbf{Motion Direction} & Prompts that involve control over motion direction.    & \textit{\makecell{flying counter clockwise around a large yacht;\\ aerial sunrise shot over a town, flying forwards}}                                                \\
                          &                                                        &                                                                                                                                                                                                   \\
\textbf{Event Order}      & Prompts that involve control over the order of events. & \textit{\makecell{an old man shakes hands with another \\ man and then they hug each other;\\ a guy slices potatoes and then adds \\ them to a bowl of heavy cream}} \\ \bottomrule
\end{tabular}
$}
\end{table*}

==> tables/temporal_content.tex <==
\begin{table*}[t]
\centering
\caption{Descriptions and examples of temporal categories under the ``major content" aspect.}
\label{tab:temporal_content}
\resizebox{\textwidth}{!}{$
\begin{tabular}{lll}
\toprule
Category                 & \multicolumn{1}{c}{Description}                                                                                                             & \multicolumn{1}{c}{Example Prompts}                                                                                                                                                 \\ \midrule
\textbf{Actions}         & Prompts that involve actions of people or animals.                                                                                          & \textit{people are dancing; a horse is eating}                                                                                                                               \\
                         &                                                                                                                                             &                                                                                                                                                                              \\
\textbf{Kinetic Motions} & Prompts that involve the motion of solid objects.                                                                                           & \textit{\makecell{the cars drove fast; \\ DNA strands spinning on screen}}                                                                      \\
                         &                                                                                                                                             &                                                                                                                                                                              \\
\textbf{Fluid Motions}   & \makecell{Prompts that involve motions of fluids or motions \\ like fluids, e.g., the deformation of objects.} & \textit{\makecell{fast speed sky and clouds when sunset; \\ the water falls down to the cliff really fast;\\ inflating balls with an air pump}} \\
                         &                                                                                                                                             &                                                                                                                                                                              \\
\textbf{Light Change}    & \makecell{Prompts from which the generated videos may involve \\ change of light or color over time.}          & \textit{\makecell{a fire is burning; star time lapse, \\ green aurora moving across the night sky}}                                             \\ \bottomrule
\end{tabular}
$}
\end{table*}

==> tables/temporal_content_attribute.tex <==
\begin{table*}[t]
\centering
\caption{Descriptions and examples of temporal categories under the ``major content'' and ``attribute control'' aspect.}
\label{tab:temporal_content}
\resizebox{\textwidth}{!}{$
\begin{tabular}{lcc}
\toprule
Category                 & \multicolumn{1}{c}{Description}                                                                                                             & \multicolumn{1}{c}{Example Prompts}                                                                                                                                                 \\ \midrule
\textit{\textbf{Aspect of major content}} \\
\textbf{Actions}         & Prompts that involve actions of people or animals.                                                                                          & \textit{people are dancing; a horse is eating}                                                                                                                               \\
                         &                                                                                                                                             &                                                                                                                                                                              \\
\textbf{Kinetic Motions} & Prompts that involve the motion of solid objects.                                                                                           & \textit{\makecell{the cars drove fast; \\ DNA strands spinning on screen}}                                                                      \\
                         &                                                                                                                                             &                                                                                                                                                                              \\
\textbf{Fluid Motions}   & \makecell{Prompts that involve motions of fluids or motions \\ like fluids, e.g., the deformation of objects.} & \textit{\makecell{fast speed sky and clouds when sunset; \\ the water falls down to the cliff really fast;\\ inflating balls with an air pump}} \\
                         &                                                                                                                                             &                                                                                                                                                                              \\
\textbf{Light Change}    & \makecell{Prompts from which the generated videos may involve \\ change of light or color over time.}          & \textit{\makecell{a fire is burning; star time lapse, \\ green aurora moving across the night sky}}                                             \\ \midrule

\textit{\textbf{Aspect of attribute control}} \\

\textbf{Speed}            & Prompts that involve control over speed.               & \textit{\makecell{the cars drove fast; \\ bees flying, slow motion shot}}                                                                                            \\
                          &                                                        &                                                                                                                                                                                                   \\
\textbf{Motion Direction} & Prompts that involve control over motion direction.    & \textit{\makecell{flying counter clockwise around a large yacht;\\ aerial sunrise shot over a town, flying forwards}}                                                \\
                          &                                                        &                                                                                                                                                                                                   \\
\textbf{Event Order}      & Prompts that involve control over the order of events. & \textit{\makecell{an old man shakes hands with another \\ man and then they hug each other;\\ a guy slices potatoes and then adds \\ them to a bowl of heavy cream}} \\ \bottomrule
\end{tabular}
$}
\end{table*}
